Dehn functions of subgroups of right-angled Artin groups

We show that for each positive integer $k$ there exist right-angled Artin groups containing free-by-cyclic subgroups whose monodromy automorphisms grow as $n^k$. As a consequence we produce examples of right-angled Artin groups containing finitely presented subgroups whose Dehn functions grow as $n^{k+2}$.

==> definitions.tex <==

\makeatletter
\newcommand*\if@single[3]{%
  \setbox0\hbox{${\mathaccent"0362{#1}}^H$}%
  \setbox2\hbox{${\mathaccent"0362{\kern0pt#1}}^H$}%
  \ifdim\ht0=\ht2 #3\else #2\fi
  }
%The bar will be moved to the right by a half of \macc@kerna, which is computed by amsmath:
\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
%If there's a superscript following the bar, then no negative kern may follow the bar;
%an additional {} makes sure that the superscript is high enough in this case:
\renewcommand*\widebar[1]{\@ifnextchar^{{\wide@bar{#1}{0}}}{\wide@bar{#1}{1}}}
%Use a separate algorithm for single symbols:
\newcommand*\wide@bar[2]{\if@single{#1}{\wide@bar@{#1}{#2}{1}}{\wide@bar@{#1}{#2}{2}}}
\newcommand*\wide@bar@[3]{%
  \begingroup
  \def\mathaccent##1##2{%
%If there's more than a single symbol, use the first character instead (see below):
    \if#32 \let\macc@nucleus\first@char \fi
%Determine the italic correction:
    \setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
    \setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
    \dimen@\wd\tw@
    \advance\dimen@-\wd\z@
%Now \dimen@ is the italic correction of the symbol.
    \divide\dimen@ 3
    \@tempdima\wd\tw@
    \advance\@tempdima-\scriptspace
%Now \@tempdima is the width of the symbol.
    \divide\@tempdima 10
    \advance\dimen@-\@tempdima
%Now \dimen@ = (italic correction / 3) - (Breite / 10)
    \ifdim\dimen@>\z@ \dimen@0pt\fi
%The bar will be shortened in the case \dimen@<0 !
    \rel@kern{0.6}\kern-\dimen@
    \if#31
      \overline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
      \advance\dimen@0.4\dimexpr\macc@kerna
%Place the combined final kern (-\dimen@) if it is >0 or if a superscript follows:
      \let\final@kern#2%
      \ifdim\dimen@<\z@ \let\final@kern1\fi
      \if\final@kern1 \kern-\dimen@\fi
    \else
      \overline{\rel@kern{-0.6}\kern\dimen@#1}%
    \fi
  }%
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
%The following initialises \macc@kerna and calls \mathaccent:
  \if#31
    \macc@nested@a\relax111{#1}%
  \else
%If the argument consists of more than one symbol, and if the first token is
%a letter, use that letter for the computations:
    \def\gobble@till@marker##1\endmarker{}%
    \futurelet\first@char\gobble@till@marker#1\endmarker
    \ifcat\noexpand\first@char A\else
      \def\first@char{}%
    \fi
    \macc@nested@a\relax111{\first@char}%
  \fi
  \endgroup
}
\makeatother

%%% a variant of 'proof' environment, to use with \tag*{$\qed$} instead of \qedhere. Works well with multline*
\makeatletter
\newenvironment{proof*}[1][\proofname]{\par
%  \pushQED{\qed}% <--- remove the QED business
  \normalfont \topsep6\p@\@plus6\p@\relax
  \trivlist
  \item[\hskip\labelsep
        \itshape
    #1\@addpunct{.}]\ignorespaces
}{%
%  \popQED% <--- remove the QED business
  \endtrivlist\@endpefalse
}
%\renewcommand\qedhere{} % to ensure code portability
\makeatother

\newcommand{\tinyb}[1]{\scalebox{0.85}{{\normalsize #1}}}

\newtheorem{thm}{Theorem}[section]
\newtheorem{prop}[thm]{Proposition}
\newtheorem{cor}[thm]{Corollary}
\newtheorem*{cora}{Corollary A}
\newtheorem{claim}[thm]{Claim}
\newtheorem{lem}[thm]{Lemma}
\newtheorem*{thma}{Theorem A}
\newtheorem*{thmb}{Theorem B}
\newtheorem*{lgthm}{Levitt's Growth Theorem}

\theoremstyle{definition}
\newtheorem{defi}[thm]{Definition}

%\theoremstyle{remark}
\newtheorem{rem}[thm]{Remark}
\newtheorem{example}[thm]{Example}
\newtheorem{que}{Question}



%\newcommand{\preceqq}{\mathrel{\substack{\prec\\[-.05em]=}}}

\newcommand{\preceqq}{\mathrel{\mathpalette\preceqqi\relax}}
\newcommand{\preceqqi}[2]{\vcenter{\offinterlineskip\lineskip1pt\hbox{$#1\prec$}\hbox{$#1=$}}}

\newcommand{\succeqq}{\mathrel{\mathpalette\succeqqi\relax}}
\newcommand{\succeqqi}[2]{\vcenter{\offinterlineskip\lineskip1pt\hbox{$#1\succ$}\hbox{$#1=$}}}



\newcommand{\pn}{\phi^n}
\newcommand{\pu}{\phi^{-n}}
\newcommand{\phii}{\phi^{-1}}
%\newcommand{\pr}{\preccurlyeq}
\newcommand{\pr}{\preceq}
\newcommand{\prq}{\preceqq}
%\newcommand{\su}{\succcurlyeq}
\newcommand{\su}{\succeq}
\newcommand{\suq}{\succeqq}
\newcommand{\Area}{\operatorname{Area}}
\newcommand{\A}{\mathcal A}
\newcommand{\B}{\mathcal B}
\newcommand{\T}{\mathcal T}
\newcommand{\Z}{\mathbb Z}
\newcommand{\C}{\mathbb C}
\newcommand{\N}{\mathbb N}
\newcommand{\R}{\mathbb R}
\newcommand{\gr}{\operatorname{gr}}
\newcommand{\ov}{\widebar}
\newcommand{\overbar}{\ov}
\newcommand{\bei}{\bar e_i}
\newcommand{\eps}{\varepsilon}
\newcommand{\End}{\operatorname{End}}
\newcommand{\Aut}{\operatorname{Aut}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\Card}{\operatorname{Card}}
\newcommand{\Sym}{\operatorname{Sym}}
\newcommand{\Id}{\operatorname{Id}}
\newcommand{\id}{\operatorname{id}}
\newcommand{\rk}{\operatorname{rank}}
\newcommand{\Lk}{\operatorname{Lk}}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\Ker}{\operatorname{Ker}}
\newcommand{\Vertices}{\operatorname{Vertices}}
\newcommand{\Edges}{\operatorname{Edges}}




\tikzset{->-/.style={decoration={
  markings,
  mark=at position #1 with {\arrow{Stealth[length=7pt,width=4.67pt]}}},postaction={decorate}}}
	
\tikzset{mapping/.style={decoration={
  markings,
  mark=at position #1 with {\arrow{Classical TikZ Rightarrow[length=3pt]}}},postaction={decorate}}}

	
%\tikzset{middlearrow/.style={
%        decoration={markings,
%            mark= at position 0.5 with {\arrow{#1}} ,
%        },
%        postaction={decorate}
%    }
%}
	

